SPFA: SFA on Multiple Persistent Faults

For classical fault analysis, a transient fault is required to be injected during runtime, e.g., only at a specific round. Instead, Persistent Fault Analysis (PFA) introduces a powerful class of fault attacks that allows for a fault to be present throughout the whole execution. One limitation of original PFA as introduced by Zhang et al. at CHES'18 is that the faulty values need to be known to the adversary. While this was addressed at a follow-up work at CHES'20, the solution is only applicable to a single faulty value. Instead, we use the potency of Statistical Fault Analysis (SFA) in the persistent fault setting, presenting Statistical Persistent Fault Analysis (SPFA) as a more general approach of PFA. As a result, any or even a multitude of unknown faults that cause an exploitable bias in the targeted round can be used to recover the cipher's secret key. Indeed, the undesired faults in the other rounds that occur due the persistent nature of the attack converge to a uniform distribution as required by SFA. We verify the effectiveness of our attack against LED and AES.

==> sections/background.tex <==
%!TEX root = ../main.tex
%\section{Related Work}
%\label{pf::sec::related_work}

 




%\subsection{Brief Overview of AES}
%\label{pf::sec::background::aes}
%This section provides a short overview of the AES block cipher, for a detailed description cp. \cite{design:aes_nsa}. 
%We analyse AES in its most common configuration with a block and key size of 128 bit.
%In this configuration, an AES encryption takes $10$ rounds. 
%Both key and plaintext are arranged in a 4$\times$4-byte state matrix.
%First, the key expansion step computes the $11$ subkeys, one for each round and another for the additional introductory key addition step.
%In addition to the key expansion, AES consists of four main components: SubBytes, ShiftRows, MixColumns, and AddRoundKey.
%In SubBytes (SB), each byte of the state is exchanged with its corresponding SBox entry.
%ShiftRows (SR) rotates the rows of the state by a fixed amount of entries to the left.  MixColumns (MC) multiplies each column of the state with a matrix M and stores the result back in the same column.
%Finally, the AddRoundKey (AK) step adds the corresponding subkey bytewise to the state matrix via exclusive-or. 
%With exception of the final round, where the MC operation is omitted, in each round, the state is successively manipulated by SubBytes, ShiftRows, MixColumns and AddRoundKey.
%In the end, the final state makes the ciphertext. 



